The Adversarial Resilience Learning Architecture for AI-based Modelling, Exploration, and Operation of Complex Cyber-Physical Systems

Modern algorithms in the domain of Deep Reinforcement Learning (DRL) demonstrated remarkable successes; most widely known are those in game-based scenarios, from ATARI video games to Go and the StarCraft~\textsc{II} real-time strategy game. However, applications in the domain of modern Cyber-Physical Systems (CPS) that take advantage a vast variety of DRL algorithms are few. We assume that the benefits would be considerable: Modern CPS have become increasingly complex and evolved beyond traditional methods of modelling and analysis. At the same time, these CPS are confronted with an increasing amount of stochastic inputs, from volatile energy sources in power grids to broad user participation stemming from markets. Approaches of system modelling that use techniques from the domain of Artificial Intelligence (AI) do not focus on analysis and operation. In this paper, we describe the concept of Adversarial Resilience Learning (ARL) that formulates a new approach to complex environment checking and resilient operation: It defines two agent classes, attacker and defender agents. The quintessence of ARL lies in both agents exploring the system and training each other without any domain knowledge. Here, we introduce the ARL software architecture that allows to use a wide range of model-free as well as model-based DRL-based algorithms, and document results of concrete experiment runs on a complex power grid.

==> sections/Architecture/environment.tex <==
\subsection{ARL-Environment}
\label{sec:arl-software-architecture-environment}
% Environment Erklärung
% Mosaik was ist es? Wofür brauchen wir es?

Environments serve as an interface between a simulator or several simulators combined as on co-simulation and the agents. The agents communicate with the environment via the internal simulation. Since the environment for an experiment is always the same, it is instantiated by each RunGovernor for each internal simulation. By using the environment as an interface the underlying (co-)simulation can be exchanged. The environment then only offers a set of sensors and actuators and an information if the environment is terminated. The reduction to sensors and actuators provides the desired domain independence. Both sensors and actuators have an approved value range. Sensors also have a sensor value, while actuators receive a setpoint. The environment collects the actions of the agents and transfers them to the simulation and executes a simulation step. Subsequently, the new sensor values are returned to the agents. 

==> sections/Architecture/simulator.tex <==

\subsection{ARL-Simulator}
\label{sec:arl-software-architecture-simulator}
% Wie funktionieren die Simulatoren
% Bezug zu Env

The simulation component is the internal execution environment. A simulation consists of the acting agents and an environment that provides the simulators. The simulation is initialized by a RunGovernor, which combines the agents with the environment according to the experiment run and configures the simulation. Sensor information as well as the agent output including the reward is sent to the RunGovernor via the ZeroMQ bus, which stores it so that an analysis of the agent steps is possible. 
